Sliced Slices: Separating Data and Control Influences

Backward slicing has been used extensively in program understanding, debugging and scaling up of program analysis. For large programs, the size of the conventional backward slice is about 25% of the program size. This may be too large to be useful. Our investigations reveal that in general, the size of a slice is influenced more by computations governing the control flow reaching the slicing criterion than by the computations governing the values relevant to the slicing criterion. We distinguish between the two by defining data slices and control slices both of which are smaller than the conventional slices which can be obtained by combining the two. This is useful because for many applications, the individual data or control slices are sufficient. Our experiments show that for more than 50% of cases, the data slice is smaller than 10% of the program in size. Besides, the time to compute data or control slice is comparable to that for computing the conventional slice.

==> relatedwork.tex <==
\section{Related Work}
After the introduction of slicing by Weiser~\cite{PROGRAM_SLICING}, 
there has been different variations of the same . 
Forward slicing~\cite{FORWARD_SLICING} and Chopping~\cite{CHOPPING} are the notables ones which compute different set of statements by considering
effects in only forward direction or those which are impacted by a given
criteria in forward direction and for another criteria in backward direction. But both of these still talk about control and data impact in a 
tightly coupled manner.
Dynamic slice~\cite{DYNAMIC_SLICING} computes a 
a subset of program statements which affect a slicing criteria  in a particular run of the program. This also does not talk about separating
data and control influences.
Assertion slicing~\cite{PRECOND_SLICING, WP_SLICING, ASSERTION_SLICING} 
is a technique which computes set of statements which
are sufficient to ensure a post condition 
or which get executed
from a given pre condition. But these also can not be used in getting 
a {\em data slice}. Other than these, to the best of our knowledge, there
is no work which talks about separating data and control influences.


